Automated control and optimisation of laser driven ion acceleration

The interaction of relativistically intense lasers with opaque targets represents a highly non-linear, multi-dimensional parameter space. This limits the utility of sequential 1D scanning of experimental parameters for the optimisation of secondary radiation, although to-date this has been the accepted methodology due to low data acquisition rates. High repetition-rate (HRR) lasers augmented by machine learning present a valuable opportunity for efficient source optimisation. Here, an automated, HRR-compatible system produced high fidelity parameter scans, revealing the influence of laser intensity on target pre-heating and proton generation. A closed-loop Bayesian optimisation of maximum proton energy, through control of the laser wavefront and target position, produced proton beams with equivalent maximum energy to manually-optimized laser pulses but using only 60% of the laser energy. This demonstration of automated optimisation of laser-driven proton beams is a crucial step towards deeper physical insight and the construction of future radiation sources.

==> authors.tex <==

\author{B. Loughran}
    \affiliation{School of Maths and Physics, Queen's University Belfast, University Road, Belfast, N. Ireland, U. K.}
\author{M. J. V. Streeter}
    \affiliation{School of Maths and Physics, Queen's University Belfast, University Road, Belfast, N. Ireland, U. K.}
\author{O. C. Ettlinger}
    \affiliation{Blackett Laboratory, Imperial College London, South Kensington Campus, London, U. K.}
\author{M. Balcazar}
    \affiliation{Center for Ultrafast Optical Science, University of Michigan Engineering, 1221 Beal Ave., Ann Arbor, Michigan, U. S. A}
\author{M. Borghesi}
    \affiliation{School of Maths and Physics, Queen's University Belfast, University Road, Belfast, N. Ireland, U. K.}
\author{N. Bourgeois}
    \affiliation{Central Laser Facility, STFC Rutherford Appleton Laboratory, Harwell Campus, Didcot, U. K.}
\author{C.~B.~Curry}
    \affiliation{SLAC National Accelerator Laboratory, 2575 Sand Hill Road, Menlo Park, California, U. S. A.}
\author{S. Dann}
    \affiliation{Central Laser Facility, STFC Rutherford Appleton Laboratory, Harwell Campus, Didcot, U. K.}
\author{S. DiIorio}
    \affiliation{Center for Ultrafast Optical Science, University of Michigan Engineering, 1221 Beal Ave., Ann Arbor, Michigan, U. S. A}
\author{N. P. Dover}
    \affiliation{Blackett Laboratory, Imperial College London, South Kensington Campus, London, U. K.}
\author{T. Dzelzanis}
    \affiliation{Central Laser Facility, STFC Rutherford Appleton Laboratory, Harwell Campus, Didcot, U. K.}
\author{V. Istokskaia}
    \affiliation{ELI Beamlines, Za Radnic\'{i} 835, 252 41 Doln\'{i}  B\u{r}e\u{z}any, Czech Republic}
\author{M.~Gauthier}
    \affiliation{SLAC National Accelerator Laboratory, 2575 Sand Hill Road, Menlo Park, California, U. S. A.}
\author{L. Giuffrida}
    \affiliation{ELI Beamlines, Za Radnic\'{i} 835, 252 41 Doln\'{i}  B\u{r}e\u{z}any, Czech Republic}
\author{G.~D.~Glenn}
    \affiliation{SLAC National Accelerator Laboratory, 2575 Sand Hill Road, Menlo Park, California, U. S. A.}
\author{S.~H.~Glenzer}
    \affiliation{SLAC National Accelerator Laboratory, 2575 Sand Hill Road, Menlo Park, California, U. S. A.}
\author{R. Gray}
    \affiliation{Department of Physics, University of Strathclyde, 16 Richmond Street, Glasgow, U. K.}
\author{A. Hamad}
    \affiliation{Central Laser Facility, STFC Rutherford Appleton Laboratory, Harwell Campus, Didcot, U. K.}
\author{G. S. Hicks}
    \affiliation{Blackett Laboratory, Imperial College London, South Kensington Campus, London, U. K.}
\author{M. King}
    \affiliation{Department of Physics, University of Strathclyde, 16 Richmond Street, Glasgow, U. K.}
\author{D. Margarone}
    \affiliation{School of Maths and Physics, Queen's University Belfast, University Road, Belfast, N. Ireland, U. K.}
\author{O. McCusker}
    \affiliation{School of Maths and Physics, Queen's University Belfast, University Road, Belfast, N. Ireland, U. K.}
\author{P. McKenna}
    \affiliation{Department of Physics, University of Strathclyde, 16 Richmond Street, Glasgow, U. K.}
\author{Z. Najmudin}
    \affiliation{Blackett Laboratory, Imperial College London, South Kensington Campus, London, U. K.}
\author{C.~Parisua{\~{n}}a}
    \affiliation{SLAC National Accelerator Laboratory, 2575 Sand Hill Road, Menlo Park, California, U. S. A.}
    \affiliation{Department of Mechanical Engineering, Stanford University, Stanford, California 94305, USA}
\author{D. Symes}
    \affiliation{Central Laser Facility, STFC Rutherford Appleton Laboratory, Harwell Campus, Didcot, U. K.}
\author{A. G. R. Thomas}
    \affiliation{Center for Ultrafast Optical Science, University of Michigan Engineering, 1221 Beal Ave., Ann Arbor, Michigan, U. S. A}
\author{F.~Treffert}
    \affiliation{SLAC National Accelerator Laboratory, 2575 Sand Hill Road, Menlo Park, California, U. S. A.}
\author{N. Xu}
    \affiliation{Blackett Laboratory, Imperial College London, South Kensington Campus, London, U. K.}
\author{C. A. J. Palmer}
    \email[Correspondence email address: ]{c.palmer@qub.ac.uk}% Your name
    \affiliation{School of Maths and Physics, Queen's University Belfast, University Road, Belfast, N. Ireland, U. K.}



==> format.tex <==
\usepackage[english]{babel}
\usepackage[utf8]{inputenc}
\usepackage[colorinlistoftodos, color=green!40, prependcaption]{todonotes}
\input{preamble}

%\setlength{\marginparwidth}{2.5cm}
\usepackage{units}
\usepackage{siunitx}
\usepackage[colorlinks = true, linkcolor = blue,
            urlcolor  = blue,citecolor = blue,
            anchorcolor = blue]{hyperref}% add hypertext capabilities
\usepackage[noabbrev]{cleveref}
\usepackage[dvipsnames]{xcolor}
\usepackage{todonotes}
\renewcommand{\d}[2]{\frac{\mbox{d} #1}{\mbox{d} #2}} % for derivatives
\newcommand{\dd}[2]{\frac{\mbox{d}^2 #1}{\mbox{d} #2^2}} % for double derivatives
\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}} % for partial derivatives
\newcommand{\avg}[1]{\left\langle #1 \right\rangle} % for average
\newcommand{\abs}[1]{\left\lvert #1 \right\rvert} % for absolute

\newcommand{\TMP}[1]{\textcolor{red}{#1}}

\bibliographystyle{apsrev4-1}

